Spatial homogeneity learning for spatially correlated functional data with application to COVID-19 Growth rate curves

We study the spatial heterogeneity effect on regional COVID-19 pandemic timing and severity by analyzing the COVID-19 growth rate curves in the United States. We propose a geographically detailed functional data grouping method equipped with a functional conditional autoregressive (CAR) prior to fully capture the spatial correlation in the pandemic curves. The spatial homogeneity pattern can then be detected by a geographically weighted Chinese restaurant process prior which allows both locally spatially contiguous groups and globally discontiguous groups. We design an efficient Markov chain Monte Carlo (MCMC) algorithm to simultaneously infer the posterior distributions of the number of groups and the grouping configuration of spatial functional data. The superior numerical performance of the proposed method over competing methods is demonstrated using simulated studies and an application to COVID-19 state-level and county-level data study in the United States.

==> plot/Walltime_summary_simulated_data_lambda.tex <==
% latex table generated in R 3.5.1 by xtable 1.8-3 package
% Sun Mar 10 20:00:35 2019
\begin{table}[ht]
\centering
\begin{tabular}{rrrrr}
  \toprule
  $\lambda$ & Joint Normal & Sufficient Reduction & Adaptive Rej. Sampling & JAGS \\ 
  \midrule
  $25$ & 537.8 & 255.2 & 6094.9 & 8.5 \\
  $50$ & 611.4 & 293.7 & 6981.5 & 9.1 \\
  $100$ & 891.2 & 377.6 & 9003.0 & 14.8 \\
  \bottomrule
\end{tabular}
\caption[Average Wall Time, over $\lambda$, for Standard Simulated Data]{Average wall Time (in seconds) for the standard simulated data for each $\lambda$.} 
\label{tbl2:walltime_simulated_data_lambda}
\end{table}
